SAR: Learning Global Item-Space Matching and Geometry-Aware Placement Ranking for Buffered Online 3D Bin Packing

Online 3D bin packing with a bounded buffer requires irreversible item-selection and placement decisions under limited knowledge of future arrivals. Feasibility alone is insufficient, as feasible actions can produce different residual-space structures and subsequent packing opportunities. A central architectural question is how to allocate spatial reasoning between item selection and placement evaluation. We propose Spatial Affordance Retrieval (SAR), a novel learning-based framework that coordinates global item-space matching with geometry-aware placement ranking. A voxel-token spatial encoder represents 3D container occupancy, enabling a picker to match buffered items to the residual space without requiring item-specific placement proposals as inputs. After item selection, a loader ranks feasible rotation-position candidates using candidate geometry, local geometric features (LGF), and inter-candidate comparison, without directly accessing global spatial tokens. The feasible candidate set connects the two stages, which are jointly optimized under a shared long-horizon packing return. On the Random, JD, and SF datasets, the best SAR variants improve utilization over the strongest evaluated online baselines by 0.96-4.20 percentage points under the no-buffer setting (K=1). With a buffer (K=5), the best utilization rates across SAR variants reach 93.55%, 91.04%, and 90.41%, respectively. Ablations support the complementary roles of global item-space matching and geometry-aware placement evaluation, counterfactual analysis suggests that learned item selection favors greater future packing potential, and experiments demonstrate compatibility with multiple candidate generators.

==> tab2.tex <==
%
\caption{Performance of SAR under different settings. All experiments were set $N_{\mathrm{ori}}=6$ and EV.}
\label{table2}
\setlength{\tabcolsep}{0.8pt}
\begin{tabular*}{\tblwidth}{@{\extracolsep{\fill}}ccccccccccc@{}}
\toprule
  & & \multicolumn{3}{c}{$R=10$} & \multicolumn{3}{c}{$R=30$} & \multicolumn{3}{c}{$R=50$} \\
  \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
  $\mathcal{D}$ & $K$ & util.$\uparrow$ & std.$\downarrow$ & num. & util.$\uparrow$ & std.$\downarrow$ & num. & util.$\uparrow$ & std.$\downarrow$ & num. \\
  \midrule
  1 & 1 & 88.46 & 4.80 & 35.17 & 87.93 & 4.80 & 34.95 & 87.60 & 5.05 & 34.85 \\
  1 & 3 & 91.61 & 3.92 & 36.91 & 91.69 & 3.56 & 37.89 & 91.21 & 4.25 & 37.45 \\
  1 & 5 & 92.54 & 4.14 & 37.68 & 93.69 & 3.88 & 37.99 & 93.60 & 3.44 & 38.38 \\
  2 & 5 & 90.13 & 4.91 & 25.13 & 91.80 & 4.75 & 25.93 & 90.21 & 5.08 & 25.17 \\
  3 & 5 & 89.30 & 5.35 & 19.90 & 88.64 & 5.12 & 20.29 & 88.37 & 4.94 & 21.68 \\
  \bottomrule
\end{tabular*}


==> tab3.tex <==
%
\caption{Ablation study of model components. All
experiments were set $K=3,R=10,N_{\mathrm{ori}}=6,\mathcal{D}_1$, and EMS.}
\label{table3}
\setlength{\tabcolsep}{2pt}
\begin{tabular*}{\tblwidth}{@{\extracolsep{\fill}}lrrrrrr@{}}
\toprule
Method & util.$\uparrow$ & $\Delta$ & std.$\downarrow$ & $\Delta$ & num. & $\Delta$ \\
\midrule
Full & 90.63 & -- & 4.69 & -- & 36.42 & -- \\
w/o FFN & 90.13 & -0.50 & 5.12 & 0.43 & 36.34 & -0.08 \\
w/o LGF & 87.93 & -2.70 & 5.07 & 0.38 & 35.68 & -0.74 \\
w/o ST & 84.22 & -6.41 & 7.72 & 3.03 & 31.97 & -4.45 \\
w/o Picker & 87.77 & -2.86 & 5.74 & 1.05 & 34.93 & -1.49 \\
w/o Loader & 62.85 & -27.78 & 12.49 & 7.80 & 26.39 & -10.03 \\
\bottomrule
\end{tabular*}

